W &gamma; production in vector boson fusion at NLO in QCD

The next-to-leading order QCD corrections to W gamma production in association with two jets via vector boson fusion are calculated, including the leptonic decay of the W with full off-shell effects and spin correlations. The process lends itself to a test of quartic gauge couplings. The next-to-leading order corrections reduce the scale uncertainty significantly and show a non-trivial phase space dependence.

==> Makefile <==
MAIN_SRC = EWWAjj_short

ARCHFLG  = $(shell if test `uname -m` == "x86_64" || \
	test `uname -m` == "i686"; then echo "ghostview"; \
	else echo "preview"; fi) 

MAIN:
		latex $(MAIN_SRC).tex
		bibtex $(MAIN_SRC)
		latex $(MAIN_SRC).tex
		latex $(MAIN_SRC).tex
		dvips $(MAIN_SRC).dvi
		ps2pdf $(MAIN_SRC).ps $(MAIN_SRC).pdf

preview:
	 	$(MAKE)
		ps2pdf $(MAIN_SRC).ps $(MAIN_SRC).pdf
		open -a Preview $(MAIN_SRC).pdf

ghostview: 
	 	$(MAKE)
		gv -antialias $(MAIN_SRC).ps &

gv:
		$(MAKE) $(ARCHFLG)

pdf: 
		$(MAKE) 
		ps2pdf $(MAIN_SRC).ps $(MAIN_SRC).pdf
		zip $(MAIN_SRC)pdf.zip $(MAIN_SRC).pdf

feyn:


tar:	         
	        $(MAKE)  
		ps2pdf $(MAIN_SRC).ps $(MAIN_SRC).pdf
	        tar cvf $(MAIN_SRC).tar $(MAIN_SRC).pdf $(MAIN_SRC).tex Makefile distributions

clean:
		rm -f *.log *.1 *.t1 $(MAIN_SRC).pdf $(MAIN_SRC).ps *.aux *.dvi *~
		rm -f *.toc *.lof $(MAIN_SRC).tar.gz *.end

